RefRec: Pseudo-labels Refinement via Shape Reconstruction for Unsupervised 3D Domain Adaptation

Unsupervised Domain Adaptation (UDA) for point cloud classification is an emerging research problem with relevant practical motivations. Reliance on multi-task learning to align features across domains has been the standard way to tackle it. In this paper, we take a different path and propose RefRec, the first approach to investigate pseudo-labels and self-training in UDA for point clouds. We present two main innovations to make self-training effective on 3D data: i) refinement of noisy pseudo-labels by matching shape descriptors that are learned by the unsupervised task of shape reconstruction on both domains; ii) a novel self-training protocol that learns domain-specific decision boundaries and reduces the negative impact of mislabelled target samples and in-domain intra-class variability. RefRec sets the new state of the art in both standard benchmarks used to test UDA for point cloud classification, showcasing the effectiveness of self-training for this important problem.

==> sections/01-related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Unsupervised Domain Adaptation (UDA)}
\label{sec:uda}
Unsupervised Domain Adaptation aims at reducing the need of large amounts of annotated data. The key idea is to learn distinctive and powerful features in the source domain and exploit such representation in the target domain. A remarkable amount of work has been conducted for image classification \cite{ganin2015, Bousmalis2016, Long2017, NIPS2016_ac627ab1, Sun2016DeepCC, Tzeng2017, Tzeng2014DeepDC, Li2017RevisitingBN}, semantic segmentation \cite{bdl,  adaptsegnet, maxsquare, pmlr-v80-hoffman18a, DCAN,  ltir} and object detection \cite{Chen2018,  Wang_2019_CVPR, Wang_2019_CVPR, Wang_2019, Saito2019}.
The most common approach to tackle UDA is to minimize the discrepancy between domains to obtain domain-invariant features, so that the same classifier can be deployed in both domains. Alignment in feature space can be achieved by forcing features from both domain to have similar statistics, as done in \cite{Long2017, NIPS2016_ac627ab1}. Another interesting line of research, instead, casts domain alignment as a min-max problem, exploiting adversarial training to attain such alignment. For example, Tzeng et al. \cite{Tzeng2017} introduced a domain confusion loss to obtain  features indistinguishable across domains.
Ganin et al. \cite{ganin2015} try to learn domain invariant representations in an adversarial way by back-propagating the reverse gradients of the domain classifier.
All these methods are meant to work with images and do not explore any variations or extensions to  exploit 3D data. In this work, instead, we turn our attention on 3D data and focus on their peculiar properties to design an effective domain adaptation methodology. 



\subsection{Unsupervised 3D Domain Adaptation}
\label{subsec:da_pcd}

Only few papers discuss Unsupervised Domain Adaptation for point cloud classification. Among these, PointDAN \cite{qin2019pointdan} is a seminal work that proposes to adapt a classical 2D domain adaptation approach to the 3D world. Specifically, they focus on the alignment of both local and global features, building their framework upon the popular Maximum Classifier Discrepancy (MCD) \cite{Saito2018MaximumCD} for global feature alignment.
Differently, \cite{alliegro2021joint,achituve2021self} leverage on Self-supervised learning (SSL) to learn simultaneously distinctive features for both the source and target domains.
Similarly, \cite{alliegro2021joint} also relays on SSL, and introduces a novel pretext task to learn strong features for the target domain as well.
In this work, we take one step further and present an unsupervised domain adaptation method based on \pl{} that exploits a shape reconstruction task to refine them. 


\subsection{Deep Learning for Point Clouds Reconstruction}
\label{subsec:ssl_pcd}
With the recent advances in deep learning several methods for point cloud reconstruction have been suggested.  A seminal work in this area \cite{Achlioptas2018LearningRA} proposes 
a new auto-encoder architecture for point clouds using the permutation invariant operator introduced in \cite{qi2017pointnet}. AtlasNet \cite{groueix2018} and FoldingNet \cite{yang2018foldingnet} propose a \textit{plane-folding} decoder to learn to deform points sampled from a plane in order to reconstruct the input surface. TearingNet \cite{pang2021tearingnet} takes inspiration from \cite{yang2018foldingnet,groueix2018} and present a \textit{tearing} module to cut regular 2D patch with holes, or into several parts, to preserve the point cloud topology. In \cite{chen2019unpaired}, the authors reconstruct the point clouds by training a generative adversarial network (GAN) on the latent space of unpaired clean synthetic and occluded real point clouds. We take inspiration from the finding of \cite{Achlioptas2018LearningRA} and leverage the expressive power of point cloud auto-encoders to pre-train our shape classifier and learn a global shape descriptor deployed for \pl{} refinement.


==> sections/04-conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we improved the state of the art in UDA for point cloud classifications. We showed how solving 3D UDA by means of \st{} with supervision from robust \pl{} is a superior paradigm with respect to the established way of tackling it by multi-task learning. Key contributions we make are effective ways to refine \pl{}, offline and online, by leveraging shape descriptors learned to solve shape reconstruction on both domains, as well as a carefully designed \st{} protocol based on domain-specific classification heads and improved supervision by an evolving mean teacher. We hope our results will call for more explorations around the use of \pl{} and \st{} in this emerging area of research. 
In future for future work, we plan to investigate novel methods to perform the warm-up step using metric learning to construct a more discriminative feature space.

\section{Acknowledgment}
The authors would like to thank Injenia Srl for supporting this research.
